FisheyeDistanceNet: Self-Supervised Scale-Aware Distance Estimation using Monocular Fisheye Camera for Autonomous Driving

Fisheye cameras are commonly used in applications like autonomous driving and surveillance to provide a large field of view ($>180^{\circ}$). However, they come at the cost of strong non-linear distortions which require more complex algorithms. In this paper, we explore Euclidean distance estimation on fisheye cameras for automotive scenes. Obtaining accurate and dense depth supervision is difficult in practice, but self-supervised learning approaches show promising results and could potentially overcome the problem. We present a novel self-supervised scale-aware framework for learning Euclidean distance and ego-motion from raw monocular fisheye videos without applying rectification. While it is possible to perform piece-wise linear approximation of fisheye projection surface and apply standard rectilinear models, it has its own set of issues like re-sampling distortion and discontinuities in transition regions. To encourage further research in this area, we will release our dataset as part of the WoodScape project \cite{yogamani2019woodscape}. We further evaluated the proposed algorithm on the KITTI dataset and obtained state-of-the-art results comparable to other self-supervised monocular methods. Qualitative results on an unseen fisheye video demonstrate impressive performance https://youtu.be/Sgq1WzoOmXg.

==> img/failure_case/failure_case.tex <==
\newcommand{\turnheightnew}{0.25\columnwidth}
\centering

\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

{\rotatebox{90}{\hspace{0mm}}} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000555_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000879_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000294_cropped.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000603_cropped.jpg}\\

{\rotatebox{90}{\hspace{0mm}\scriptsize}} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000555_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000879_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000294_box.jpg} &
\includegraphics[height=\turnheightnew]{img/failure_case/0000000603_box.jpg} \\

\end{tabular}


==> img/kitti_fig/kitti_fig.tex <==
\newcommand{\turnheightnew}{0.195\columnwidth}
\centering

\begin{tabular}{@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{\hskip 2mm}c@{}}

{\rotatebox{90}{\hspace{4mm}Input}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_color.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_color.jpg}\\

{\rotatebox{90}{\hspace{0mm}\scriptsize
{Monodepth~\cite{monodepth17}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_monodepth_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_monodepth_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize
{Zhou et al.~\cite{zhou2017unsupervised}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_zhou_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_zhou_disp.jpg} \\

{\rotatebox{90}{\hspace{2mm}\scriptsize
{DDVO~\cite{Wang_2018_CVPR}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_posenet_ddvo_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_posenet_ddvo_disp.jpg} \\


{\rotatebox{90}{\hspace{2mm}\scriptsize
{GeoNet~\cite{yin2018geonet}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_geonet_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_geonet_disp.jpg} \\

{\rotatebox{90}{\hspace{0mm}\scriptsize
{Zhan et al.~\cite{zhan2018unsupervised}}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_zhan_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_zhan_disp.jpg} \\

{\rotatebox{90}{\hspace{-1mm}\scriptsize
Ranjan et al.~\cite{ranjan2019competitive}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_gan_adv_col_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_gan_adv_col_disp.jpg} \\


{\rotatebox{90}{\hspace{0mm} \scriptsize
3Net-R50~\cite{luo2018every}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_3net_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_3net_disp.jpg} \\ 

{\rotatebox{90}{\hspace{0mm} \scriptsize
EPC++ (MS) \newline \cite{luo2018every}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_epcpp_ms_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_epcpp_ms_disp.jpg} \\ 

{\rotatebox{90}{\hspace{0mm}\scriptsize
Monodepth2 M~\cite{godard2018digging}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_monodepth2_disp.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_monodepth2_disp.jpg} \\

{\rotatebox{90}{\hspace{3mm}\scriptsize
\textbf{Ours M}}} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0084_sync_283_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0036_sync_64_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0046_sync_110_ours_depth.jpg} &
\includegraphics[height=\turnheightnew]{img/kitti_fig/2011_09_26_drive_0106_sync_43_ours_depth.jpg} \\

\end{tabular}


==> results/kitti_ablation.tex <==
\begin{table*}[t!]
\captionsetup{singlelinecheck=false, justification=raggedright, font=footnotesize, labelsep=space}
\small
\begin{center}
	\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c}
	\hline
    Method & FS & BS & SR & CSDCL & Abs Rel & Sq Rel & RMSE & RMSE log & \cellcolor[HTML]{e8715b}$\delta < 1.25$ & \cellcolor[HTML]{e8715b}$\delta < 1.25^2$ &  \cellcolor[HTML]{e8715b}$\delta < 1.25^3$\\
    \hline\hline
    Ours & \checkmark & \checkmark & \checkmark & \checkmark & 0.117 & 0.867 & 4.739 & 0.190 & 0.869 & 0.960 & 0.982 \\
    Ours & \checkmark & \checkmark &            & \checkmark & 0.133 & 0.884 & 4.951 & 0.212 & 0.845 & 0.952 & 0.980 \\
    Ours & \checkmark &            &            & \checkmark & 0.134 & 0.929 & 5.063 & 0.215 & 0.835 & 0.947 & 0.979 \\
    Ours & \checkmark &            &            &            & 0.144 & 1.029 & 5.146 & 0.258 & 0.817 & 0.945 & 0.974 \\
    \hline
\end{tabular}
\end{center}
\caption{\textbf{Ablation study of our algorithm on the KITTI Eigen split dataset~\cite{geiger2013vision}}. Distances are capped at $80\,m$. BS, SR (ICNR), CSDCL, and DCN represent a backward sequence, super-resolution network with PixelShuffle, or sub-pixel convolution initialized to convolution NN resize (ICNR)~\cite{aitken2017checkerboard} and cross-sequence distance consistency loss, respectively. The input resolution is $640 \times 192$ pixels.}
\label{table:kittiablation}
\end{table*}
